Real-Time Target Sound Extraction

We present the first neural network model to achieve real-time and streaming target sound extraction. To accomplish this, we propose Waveformer, an encoder-decoder architecture with a stack of dilated causal convolution layers as the encoder, and a transformer decoder layer as the decoder. This hybrid architecture uses dilated causal convolutions for processing large receptive fields in a computationally efficient manner while also leveraging the generalization performance of transformer-based architectures. Our evaluations show as much as 2.2-3.3 dB improvement in SI-SNRi compared to the prior models for this task while having a 1.2-4x smaller model size and a 1.5-2x lower runtime. We provide code, dataset, and audio samples: https://waveformer.cs.washington.edu/.

==> method.tex <==

\section{Method}
% ~\cite{zhen2019deep}
For an unnoticeable latency, real-time audio systems require an algorithmic latency less than to 10 ms \cite{7952149}. Targeting such systems, we look at the target sound extraction problem in the context of streaming. While a model's causality is usually defined at sample level, in a streaming application, causality is defined at chunk level: an output chunk can only depend on the current chunk and past chunks. As a result, streaming models have an intrinsic latency equal to the duration of a single chunk. In this work, we propose a deep neural network architecture for streaming target sound extraction that operates on individual audio chunks of arbitrary duration $\tau$, where $\tau$ can be set to the maximum algorithmic latency allowed by the system.

\subsection{Streaming target sound extraction}
\label{sec:stream}
As shown in the Figure \ref{fig:top_level}, we propose a Tasnet \cite{https://doi.org/10.48550/arxiv.1711.00541} style time domain architecture that employs a mask generation network to generate an element-wise multiplicative mask in the latent space. Let $x_k \in R^{S}$ be the input audio chunk, where $S = \tau F_s$ is the chunk length in number of audio samples for a sampling rate $F_s$. In the first step, a 1d-convolution layer with stride $L$ is applied the time domain audio chunk $x_k$ to obtain the latent space representation of the input audio chunk, $y_k \in R^{E \times K}$, where $E$ is the latent space feature dimensions and $K = \frac{S}{L}$ is the chunk length in the latent space. Given a one-hot or multi-hot query vector $q^T \in \{0, 1\}^{N_c}$, where $N_c$ is the total number of classes, the problem of streaming target sound extraction can be formulating as computing the mask $m_k \in R^{E \times K}$. With the mask generation network denoted as $\mathcal{M}$, $\forall k \in \{1, 2, 3, ...\}$ estimated target audio chunk $\hat{x}_k \in R ^ S$ is computed in a streaming fashion as:
\begin{gather*}
    y_k = Conv1d(x_k) \\
    m_k = \mathcal{M}(y_k\ |\ y_{k-1}, .., y_2, y_1, q^T) \\
    \hat{x}_k = ConvTranspose1d(y_k \odot m_k)
\end{gather*}

\subsection{Efficient processing of the receptive field using dilated causal convolutions}
We employ an encoder-decoder architecture for the mask generation. The encoder is a stack of dilated causal convolution (DCC) layers \cite{https://doi.org/10.48550/arxiv.1609.03499} and the decoder is a transformer decoder \cite{https://doi.org/10.48550/arxiv.1706.03762}. The motivation for such an architecture for this problem is that, the encoder computes a \emph{contextful} representation of the input chunk, considering the previous chunks up to a certain receptive filed, and the decoder conditions the encoder output with the query vector to estimate the target mask. Recent works on transformer based models for speech separation \cite{subakan2021attention, subakan2022resource} have demonstrated the performance gains over convolution based methods \cite{luo2019conv}, but convolution based method have generally been more computationally efficient.

We attribute this gap in efficiency to the difference in the way existing transformer based architectures process the receptive filed compared to convolution based architectures. To achieve a receptive field of length $R$, owing to chunk based processing in existing transformer architectures, each chunk individually attends to all previous chunks in the receptive field resulting in $\mathcal{O}(R)$ complexity. Convolution based architectures \cite{https://doi.org/10.48550/arxiv.1609.03499, luo2019conv} implementing a stack of $M$ DCC layers with a kernel size $P$, have a receptive field equal to $(P - 1)\ 2^{M - 1}$, however, the number of operations has the complexity $\mathcal{O}(PM)$. Writing in terms of the receptive field $R$, the computational complexity of the stacked DCC layers to achieve a receptive filed of length $R$ is $\mathcal{O}(1 + \log \frac{R}{P - 1})$ = $\mathcal{O} (\log R)$, as the kernel size $P$ is usually a small constant $\geq 1$.

Hence, in our implementation, we use a stack of DCC layers as the encoder of our mask generation network. We use 10 layers and kernel size equal to 3 in our encoder, resulting a receptive field of $(3 - 1)\ .\ 2 ^ {(10 - 1)} = 1024$ samples in the latent space. With the initial input convolution stride $L$ set to be equivalent to 1 ms, receptive field of our encoder is $\approx1s$. In the figure \ref{fig:enc}, we show an example encoding of an input chunk of length 4. For chunk based streaming inference, the encoder maintains a context buffer for each DCC layer. This context is initially computed from the $\approx1s$ receptive field, and then updated dynamically after encoding each subsequent chunk. For encoding a chunk, each DCC layer is fed with the output chunk of the previous layer, left padded with the context of length twice the layer's dilation. After encoding a chunk, the context is updated with the rightmost elements of the padded input for it be used in encoding the next chunk. For each input chunk $y_k$ (output of the initial $Conv1d$ block), DCC encoder computes an encoded representation $e_k \in R^{E \times K}$. 

\subsection{Query conditioned decoding with linear attention}
Encoder output only depends on the current input chunk and the encoder buffer computed from the receptive field. To obtain the final mask, this encoded representation has to be conditioned with the query vector $q^T$. We first compute an embedding, $l \in R^{E \times 1}$, corresponding to $q^T$ using an embedding layer. The embedding layer comprises of three feed-forward sub-layers, with the hidden dimension equal to 512, and the input \& output dimensions equal to $E$. The decoder conditions the encoded chunk $e_k$ with the query embedding $l$. Motivated by the success of the transformer based architectures for speech processing tasks \cite{https://doi.org/10.48550/arxiv.2010.13154, 9413535}, we employ a transformer decoder layer for estimating the target mask, shown in \ref{fig:dec}.

Similar to \cite{2020arXiv200605712O, delcroix2022soundbeam}, we perform multiplicative query integration to compute conditioned representation: ${e_k}^\prime = e_k \odot l$. Since transformers are more computationally expensive at higher dimensionality, we first project the encoded representations, ${e_k}^\prime$ and $e_k$ to decoder dimensions $D \le E$, using 1x1 convolution layers. This results in projected encoded representations ${pe}_k, {{pe}_k}^\prime \in R^{D \times K}$. The decoded representations are then computed by passing ${{pe}_k, {pe}_k}^\prime$ to the transformer decoder layer's self-attention and cross-attention blocks, respectively, to obtain the target mask in the projected decoder space, ${pm}_k \in R^{D \times K}$. The target mask is then projected back to encoder dimensions using another 1x1 convolution layer to obtain the ${m_k}^\prime \in R^{E \times K}$. All projections include a ReLU non-linearity. Owing to this non-linearity, we observed that the projection layers affect the gradient flow to the embedding layer. To circumvent this, we add a skip connection immediately after the multiplicative query integration to the output of the projection layer to compute the final mask: $m_k = {m_k}^\prime + {e_k}^\prime$. The mask $m_k$ is then used to compute extract the target sound, as described in \ref{sec:stream}.

==> related.tex <==
\section{Related work}
{\bf Universal sound separation} Universal sound separation~\cite{kavalerov2019universal} is the task of separating a mixture of arbitrary sound types into their component sounds, regardless of the number of sounds in the mixture. This task becomes increasingly challenging as the number of possible sound types in the mixture increases. Prior work in this area have made progress by constructing an open dataset with mixtures of sounds drawn from hundreds of different classes~\cite{wisdom2021s}. Several network architectures have been proposed for the task including convolutional long short-term memory networks~\cite{kavalerov2019universal}, time-dilated convolution networks~\cite{kavalerov2019universal} based on ConvTas-Net~\cite{luo2019conv}, and Transformer networks~\cite{zadeh2019wildmix}. Further work proposed the use of embeddings learned by a sound classifier trained on a large ontology of sounds~\cite{gemmeke2017audio} to condition a separation network with additional information. Unlike these works, our work is focused on the related problem of extracting target sound classes from a mixture.

\noindent {\bf Target sound extraction.} Target source extraction refers to the task of separating one or more sounds of interest from a mixture by conditioning a source-separation model with query information or clues about the target like an embedding of an audio clip~\cite{delcroix2022soundbeam}, an image~\cite{gao2019co,xu2019recursive}, natural language text~\cite{kilgour2022text,liu2022separate}, onomatopoeic words~\cite{okamoto2022environmental}, or a one-hot sound label vector~\cite{2020arXiv200605712O}. Prior work~\cite{kong2020source,chen2022zero} has also evaluated the use of a sound event detector to detect the time when a target sound occurs in a mixture. Multiple modalities like natural language and sound samples have also been used in combination to exploit common information between them~\cite{kilgour2022text}. Although, these works are often motivated as being useful for real-time applications~\cite{liu2022separate,2020arXiv200605712O}, none of them are causal. In contrast, we design the first causal network for real-time target sound extraction of diverse sound events. 

\noindent {\bf Speech networks.}
Prior work in the domain of speech has focused on speech enhancement~\cite{wisdom2019differentiable,eskimez2022personalized,chatterjee2022clearbuds}, which is the separation of relatively structured sounds of speech from non-speech interference, speech separation~\cite{luo2019conv,luo2020dual,huang2014deep,hershey2016deep,isik2016single,yu2017permutation,wang2018voicefilter} which is the separation of all voices in a mixture, and speech selection which is the extraction of a target speaker from a mixture given clues provided to the network~\cite{tzinis2022heterogeneous,ephrat2018looking}. For the task of speech enhancement, causal networks based on a complex convolution recurrent network and a deep convolution attention U-Net have been proposed~\cite{eskimez2022personalized} to achieve real-time performance. For speech separation, Transformer networks have recently been used to achieve state-of-the-art performance due to its ability to learn short and long-term dependencies~\cite{subakan2021attention,luo2022tiny}. However, the use of Transformer networks for the task of target sound extraction remains under-explored. In this work we present the first causal Transformer model for real-time target sound extraction.
